Proceedings of the 20th International Overture Workshop

This volume contains the papers presented at the 20th International Overture Workshop, which was held in an hybrid format: online and physically at Aarhus, Denmark on 05th July 2022. This event was the latest in a series of workshops around the Vienna Development Method (VDM), the open-source project Overture, and related tools and formalisms. VDM is one of the longest established formal methods for systems development. A lively community of researchers and practitioners has grown up in academia and industry around the modelling languages (VDM-SL, VDM++, VDM-RT, CML) and tools (VDMTools, Overture, VDM VSCode extension, Crescendo, Symphony, the INTO-CPS chain, and ViennaTalk). Together, these provide a platform for work on modelling and analysis technology that includes static and dynamic analysis, test generation, execution support, and model checking. This workshop provided updates on the emerging technology of VDM/Overture, including collaboration infrastructure, collaborative modelling and co-simulation for Cyber-Physical Systems.

==> 2-Villadsen/listings/LoC_v1.tex <==
\begin{table}[]
\centering
\caption{LoC measures for the files and directories used to support VDM in VS Code\protect\footnotemark{}.}
\label{tab:LoC}
\begin{tabular}{|l|r|r|r|r|}
\hline
\textbf{Directory/File} & \textbf{Code}                     & \textbf{Comment}                 & \textbf{Blank}                   & \textbf{Total}                    \\ \hline
\multicolumn{5}{|c|}{LSP/DAP support for VDMJ}                                                                                                                        \\ \hline
dap                     & 699                               & 450                              & 186                              & 1335                              \\ \hline
json                    & 551                               & 184                              & 128                              & 863                               \\ \hline
lsp                     & 1242                              & 492                              & 257                              & 1991                              \\ \hline
rpc                     & 177                               & 137                              & 54                               & 368                               \\ \hline
vdmj                    & 1940                              & 429                              & 374                              & 2743                              \\ \hline
workspace               & 1438                              & 123                              & 251                              & 1812                              \\ \hline
\textbf{Sum}            & \textbf{6047}                     & \textbf{1815}                    & \textbf{1250}                    & \textbf{9112}                     \\ \hline
\multicolumn{5}{|c|}{VS Code Extension}                                                                                                                               \\ \hline
extension.ts            & \multicolumn{1}{l|}{150}          & \multicolumn{1}{l|}{30}          & \multicolumn{1}{l|}{34}          & \multicolumn{1}{l|}{214}          \\ \hline
package.json            & \multicolumn{1}{l|}{131}          & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{132}          \\ \hline
syntax highlight        & \multicolumn{1}{l|}{374}          & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{374}          \\ \hline
\textbf{Sum}            & \multicolumn{1}{l|}{\textbf{655}} & \multicolumn{1}{l|}{\textbf{30}} & \multicolumn{1}{l|}{\textbf{35}} & \multicolumn{1}{l|}{\textbf{720}} \\ \hline
\end{tabular}
\end{table}

==> 2-Villadsen/listings/LoC_v2.tex <==
\begin{table}[]
\centering
\caption{LoC measures for the files and directories used to support VDM in VS Code\protect\footnotemark{}.}
\label{tab:LoC}
\begin{tabular}{|l|r|r|r|r|llllll}
\cline{1-5} \cline{7-11}
\multicolumn{5}{|c|}{LSP/DAP support for VDMJ}                                               & \multicolumn{1}{l|}{} & \multicolumn{5}{c|}{VS Code Extension}                                                                                                                                                                \\ \cline{1-5} \cline{7-11} 
\textbf{Directory/File} & \textbf{Code} & \textbf{Comment} & \textbf{Blank} & \textbf{Total} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\textbf{Directory/File}} & \multicolumn{1}{r|}{\textbf{Code}} & \multicolumn{1}{r|}{\textbf{Comment}} & \multicolumn{1}{r|}{\textbf{Blank}} & \multicolumn{1}{r|}{\textbf{Total}} \\ \cline{1-5} \cline{7-11} 
dap                     & 699           & 450              & 186            & 1335           & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{extension.ts}            & \multicolumn{1}{l|}{150}           & \multicolumn{1}{l|}{30}               & \multicolumn{1}{l|}{34}             & \multicolumn{1}{l|}{214}            \\ \cline{1-5} \cline{7-11} 
json                    & 551           & 184              & 128            & 863            & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{package.json}            & \multicolumn{1}{l|}{131}           & \multicolumn{1}{l|}{0}                & \multicolumn{1}{l|}{1}              & \multicolumn{1}{l|}{132}            \\ \cline{1-5} \cline{7-11} 
lsp                     & 1242          & 492              & 257            & 1991           & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{syntax highlight}        & \multicolumn{1}{l|}{374}           & \multicolumn{1}{l|}{0}                & \multicolumn{1}{l|}{0}              & \multicolumn{1}{l|}{374}            \\ \cline{1-5} \cline{7-11} 
rpc                     & 177           & 137              & 54             & 368            & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\textbf{Sum}}            & \multicolumn{1}{l|}{\textbf{655}}  & \multicolumn{1}{l|}{\textbf{30}}      & \multicolumn{1}{l|}{\textbf{35}}    & \multicolumn{1}{l|}{\textbf{720}}   \\ \cline{1-5} \cline{7-11} 
vdmj                    & 1940          & 429              & 374            & 2743           &                       &                                              &                                    &                                       &                                     &                                     \\ \cline{1-5}
workspace               & 1438          & 123              & 251            & 1812           &                       &                                              &                                    &                                       &                                     &                                     \\ \cline{1-5}
\textbf{Sum}            & \textbf{6047} & \textbf{1815}    & \textbf{1250}  & \textbf{9112}  &                       &                                              &                                    &                                       &                                     &                                     \\ \cline{1-5}
\end{tabular}
\end{table}

==> 3-Rask/listings/LoC_v1.tex <==
\begin{table}[]
\centering
\caption{LoC measures for the files and directories used to support VDM in VS Code\protect\footnotemark{}.}
\label{tab:LoC}
\begin{tabular}{|l|r|r|r|r|}
\hline
\textbf{Directory/File} & \textbf{Code}                     & \textbf{Comment}                 & \textbf{Blank}                   & \textbf{Total}                    \\ \hline
\multicolumn{5}{|c|}{LSP/DAP support for VDMJ}                                                                                                                        \\ \hline
dap                     & 699                               & 450                              & 186                              & 1335                              \\ \hline
json                    & 551                               & 184                              & 128                              & 863                               \\ \hline
lsp                     & 1242                              & 492                              & 257                              & 1991                              \\ \hline
rpc                     & 177                               & 137                              & 54                               & 368                               \\ \hline
vdmj                    & 1940                              & 429                              & 374                              & 2743                              \\ \hline
workspace               & 1438                              & 123                              & 251                              & 1812                              \\ \hline
\textbf{Sum}            & \textbf{6047}                     & \textbf{1815}                    & \textbf{1250}                    & \textbf{9112}                     \\ \hline
\multicolumn{5}{|c|}{VS Code Extension}                                                                                                                               \\ \hline
extension.ts            & \multicolumn{1}{l|}{150}          & \multicolumn{1}{l|}{30}          & \multicolumn{1}{l|}{34}          & \multicolumn{1}{l|}{214}          \\ \hline
package.json            & \multicolumn{1}{l|}{131}          & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{132}          \\ \hline
syntax highlight        & \multicolumn{1}{l|}{374}          & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{374}          \\ \hline
\textbf{Sum}            & \multicolumn{1}{l|}{\textbf{655}} & \multicolumn{1}{l|}{\textbf{30}} & \multicolumn{1}{l|}{\textbf{35}} & \multicolumn{1}{l|}{\textbf{720}} \\ \hline
\end{tabular}
\end{table}

==> 3-Rask/listings/LoC_v2.tex <==
\begin{table}[]
\centering
\caption{LoC measures for the files and directories used to support VDM in VS Code\protect\footnotemark{}.}
\label{tab:LoC}
\begin{tabular}{|l|r|r|r|r|llllll}
\cline{1-5} \cline{7-11}
\multicolumn{5}{|c|}{LSP/DAP support for VDMJ}                                               & \multicolumn{1}{l|}{} & \multicolumn{5}{c|}{VS Code Extension}                                                                                                                                                                \\ \cline{1-5} \cline{7-11} 
\textbf{Directory/File} & \textbf{Code} & \textbf{Comment} & \textbf{Blank} & \textbf{Total} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\textbf{Directory/File}} & \multicolumn{1}{r|}{\textbf{Code}} & \multicolumn{1}{r|}{\textbf{Comment}} & \multicolumn{1}{r|}{\textbf{Blank}} & \multicolumn{1}{r|}{\textbf{Total}} \\ \cline{1-5} \cline{7-11} 
dap                     & 699           & 450              & 186            & 1335           & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{extension.ts}            & \multicolumn{1}{l|}{150}           & \multicolumn{1}{l|}{30}               & \multicolumn{1}{l|}{34}             & \multicolumn{1}{l|}{214}            \\ \cline{1-5} \cline{7-11} 
json                    & 551           & 184              & 128            & 863            & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{package.json}            & \multicolumn{1}{l|}{131}           & \multicolumn{1}{l|}{0}                & \multicolumn{1}{l|}{1}              & \multicolumn{1}{l|}{132}            \\ \cline{1-5} \cline{7-11} 
lsp                     & 1242          & 492              & 257            & 1991           & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{syntax highlight}        & \multicolumn{1}{l|}{374}           & \multicolumn{1}{l|}{0}                & \multicolumn{1}{l|}{0}              & \multicolumn{1}{l|}{374}            \\ \cline{1-5} \cline{7-11} 
rpc                     & 177           & 137              & 54             & 368            & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\textbf{Sum}}            & \multicolumn{1}{l|}{\textbf{655}}  & \multicolumn{1}{l|}{\textbf{30}}      & \multicolumn{1}{l|}{\textbf{35}}    & \multicolumn{1}{l|}{\textbf{720}}   \\ \cline{1-5} \cline{7-11} 
vdmj                    & 1940          & 429              & 374            & 2743           &                       &                                              &                                    &                                       &                                     &                                     \\ \cline{1-5}
workspace               & 1438          & 123              & 251            & 1812           &                       &                                              &                                    &                                       &                                     &                                     \\ \cline{1-5}
\textbf{Sum}            & \textbf{6047} & \textbf{1815}    & \textbf{1250}  & \textbf{9112}  &                       &                                              &                                    &                                       &                                     &                                     \\ \cline{1-5}
\end{tabular}
\end{table}

==> 3-Rask/tables/LoCCompare.tex <==
\begin{table}[htbp]
\centering
\caption{LoC measure for all IDE related files in the VS Code extension, the Emacs extension and Overture}
\label{tab:LoCCompare}
\begin{tabular}{|l|c|c|c|}
\hline
Project       & VS Code (+VDMJ)                 & Emacs                    & Overture                               \\ \hline
Lines of Code & \multicolumn{1}{r|}{1880 (+7855)} & \multicolumn{1}{r|}{349} & \multicolumn{1}{r|}{\textgreater{}63K} \\ \hline
\end{tabular}
\end{table}

==> 3-Rask/tables/LoCOverview.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[htbp]
\centering
\caption{LoC measures for the files and directories used to support VDM in VS Code\protect\footnotemark}
\label{tab:LoCOverview}
\begin{tabular}{|l|r|r|r|r|lllrrrr}
\cline{1-5} \cline{8-12}
\multicolumn{5}{|c|}{\cellcolor[HTML]{C0C0C0}SLSP/DAP support for VDMJ}                 & \textbf{} & \multicolumn{1}{l|}{\textbf{}} & \multicolumn{5}{c|}{\cellcolor[HTML]{C0C0C0}VS Code Extension}                                                                                                                                 \\ \cline{1-5} \cline{8-12} 
\textbf{Directory} & \textbf{Code} & \textbf{Comment} & \textbf{Blank} & \textbf{Total} &           & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{\textbf{Feature}} & \multicolumn{1}{r|}{\textbf{Code}} & \multicolumn{1}{r|}{\textbf{Comment}} & \multicolumn{1}{r|}{\textbf{Blank}} & \multicolumn{1}{r|}{\textbf{Total}} \\ \cline{1-5} \cline{8-12} 
dap                & 699           & 450              & 185            & 1334           &           & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{LSP client}       & \multicolumn{1}{r|}{156}           & \multicolumn{1}{r|}{16}               & \multicolumn{1}{r|}{29}             & \multicolumn{1}{r|}{201}            \\ \cline{1-5} \cline{8-12} 
json               & 635           & 184              & 139            & 958            &           & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{DAP client}       & \multicolumn{1}{r|}{54}            & \multicolumn{1}{r|}{10}               & \multicolumn{1}{r|}{15}             & \multicolumn{1}{r|}{79}             \\ \cline{1-5} \cline{8-12} 
lsp                & 1653          & 625              & 337            & 2615           &           & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{POG}              & \multicolumn{1}{r|}{460}           & \multicolumn{1}{r|}{51}               & \multicolumn{1}{r|}{96}             & \multicolumn{1}{r|}{607}            \\ \cline{1-5} \cline{8-12} 
lsp/lspx           & 169           & 44               & 30             & 243            &           & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{CT}               & \multicolumn{1}{r|}{732}           & \multicolumn{1}{r|}{105}              & \multicolumn{1}{r|}{165}            & \multicolumn{1}{r|}{1002}           \\ \cline{1-5} \cline{8-12} 
rpc                & 187           & 138              & 56             & 381            &           & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{Syntax highlight} & \multicolumn{1}{r|}{374}           & \multicolumn{1}{r|}{0}                & \multicolumn{1}{r|}{0}              & \multicolumn{1}{r|}{374}            \\ \cline{1-5} \cline{8-12} 
vdmj               & 2026          & 451              & 392            & 2869           &           & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{SLSP protocol}    & \multicolumn{1}{r|}{104}           & \multicolumn{1}{r|}{167}              & \multicolumn{1}{r|}{27}             & \multicolumn{1}{r|}{298}            \\ \cline{1-5} \cline{8-12} 
workspace          & 2655          & 641              & 545            & 3841           &           & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{\textbf{Sum}}     & \multicolumn{1}{r|}{\textbf{1880}} & \multicolumn{1}{r|}{\textbf{349}}     & \multicolumn{1}{r|}{\textbf{332}}   & \multicolumn{1}{r|}{\textbf{2561}}  \\ \cline{1-5} \cline{8-12} 
\textbf{Sum}       & \textbf{7855} & \textbf{2489}    & \textbf{1654}  & \textbf{11998} &           &                                &                                       &                                    &                                       &                                     &                                     \\ \cline{1-5}
\end{tabular}
\end{table}
\footnotetext{The LoC is counted using the ``VS Code Counter'' extension found at: \url{https://marketplace.visualstudio.com/items?itemName=uctakeoff.vscode-counter}}

==> defs.tex <==
% Custom VDM style
\lstdefinestyle{VDM}
{
  frame=single,
  basicstyle=\small\ttfamily,
  escapechar=!,
  breaklines=true,
  %basicstyle=\footnotesize\ttfamily,
  frameround=false,
  linewidth=\columnwidth,
  morekeywords={atomic,is,inv,values,dcl,forall,in,set,nil,and,let,be,st,set1,pure,nat,pre,post,map,to,of,true,false},
  moredelim={[is][keywordstyle]{@}{@}},
}

\lstdefinestyle{TraceOutput}
{
  basicstyle=\small\ttfamily,
  % breaklines=true,
  frame=single,
  captionpos=b
}

% Fixed width/right-aligned column type
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
